Bidding Games and Efficient Allocations

Richman games are zero-sum games, where in each turn players bid in order to determine who will play next [Lazarus et al.'99]. We extend the theory to impartial general-sum two player games called \emph{bidding games}, showing the existence of pure subgame-perfect equilibria (PSPE). In particular, we show that PSPEs form a semilattice, with a unique and natural \emph{Bottom Equilibrium}. Our main result shows that if only two actions available to the players in each node, then the Bottom Equilibrium has additional properties: (a) utilities are monotone in budget; (b) every outcome is Pareto-efficient; and (c) any Pareto-efficient outcome is attained for some budget. In the context of combinatorial bargaining, we show that a player with a fraction of X% of the total budget prefers her allocation to X% of the possible allocations. In addition, we provide a polynomial-time algorithm to compute the Bottom Equilibrium of a binary bidding game.

==> krt3.tex <==



\section {Introduction}
\paragraph {Bidding games.} 



Bidding games appeared earlier in the context of adding a bidding
phase to recreational board games such as Tic-Tac-Toe, Chess, Go, etc.  
These zero-sum bidding
games are known as Richman games, and were studied in a seminal paper by Lazarus et al. [16] and later by Develin
and Payne [9]. It is important to note that the 
bidding is performed with ``script money'' and that the utility of the players depend only on the payoff of the original games. 
Lazarus et als showed, among other results, a remarkable equivalence theorem
between Richman games and "random-turn" games (see also \cite {} ). Develin and Payne demonstrated that for tic-tac-toe 
a ratio of  133:123 in the initial budget between the two players is sufficient to guarantee winning.   See Related Work 
for more details on Richman games and other variations of bidding
games. 


There are two novel aspects of our work. The first is that we propose the internal bidding mechanism for mechanism 
design and demonstrate its use for 
allocation of indivisible goods to heterogeneous agents. {\it Auctionization} - adding internal auctions with script money, can be compared in spirit to 
{\it randomization} which is an important tool in game theory and mechanism design (as well as in the theory of algorithms).   
The second is the study of non zero-sum bidding games - 
we study, for the first time, bidding games with general utility functions.  
Whereas zero-sum games have a value that each player can guaranty, when
extending the definition to general-sum games we can only talk about equilibrium. Since bidding
games are extensive form games, a natural solution concept to look at is pure 
subgame-perfect equilibrium (PSPE). 
We apply our general theory to the much studied question of efficient allocation by proposing 
a mechanism based on sequential script auctions. 

\paragraph {Efficient allocations via sequential script auctions} 

Allocation of indivisible goods to heterogeneous agents has received much attention in the literature
of both economics and computer science. There are various criteria that an allocation mechanism or
protocol is expected to meet. Some of these criteria, such as efficiency or fairness, regard the final
allocation. An allocation is efficient (or Pareto-efficient) if no other allocation is weakly preferred
by all agents and strictly preferred by some. Other properties relate to the process by which the
allocation is decided, where agents’ incentives and strategies play an important role. For example,
if the allocation is based on agents reporting private information, then we would favor a mechanism
that is truthful. Similarly, if the allocation is achieved via a game or a market in which agents
participate, we would like a good allocation to be in equilibrium.
Often, the introduction of money solves much of the problems raised by indivisibility, and helps
to align agents’ incentives via a simultaneous or sequential auction. Implementing efficient allocations
without money is typically much harder.
In order to tackle this challenge, we introduce and study a variation of a sequential auction
without money. Rather, each agent has an initial endowment of “scrip money” currency that has
no value outside the game.
While allocation using scrip money has been suggested both in theory and in practice [12; 28;
6; 7], typically the setting is quite different, with many bidders and private valuations. 
We focus on a variant of such an auction that is specific to two agents with public information. 
The only paper we are aware of in a similar setting is by Huang et al. [11], which study a sequential auction of
identical items (see Related Work).
In short, in the sequential scrip auction (SSA) mechanism items are offered for sale in some
arbitrary order, and a first-price auction is held in each round. The higher bidder pays her bid to the
lower bidder, and gets to decide who takes the item (if valuations are monotone, then w.l.o.g. the
winner always takes the item). Note that the total amount of scrip money in the hands of the agents
remains the same, emphasizing that this is a bargaining mechanism, with no notion of “revenue”.

\paragraph {Our contribution}  

Here is our main result (informally stated): 
\begin {theorem} 
Given a two-players bidding game over a binary tree 
\begin {itemize} 
\item
For every allocation of initial budegets, 
the gane has a natural subgame-perfect equilibrium  
that is Pareto-efficient.  
\item
Every Pareto-efficient
outcome is achieved for some initial budget allocation. 
\item
The utility of each agent is
weakly increasing in her budget. 
\end {itemize}

\end {theorem}

It
is not hard to see that any sequential scrip auction with k items coincides with a 
bidding game over a balanced binary tree of height k.
Thus, our results immediately apply to the SSA mechanism, guarantying an efficient allocation
of items to two agents.

Our result can be applied not just to allocation problems, but also in other domains where
two agents have combinatorial preferences over outcomes, including multi-issue voting [15] and
selection of arbitrators [8].
To facilitate reading, most of the results except out main theorem are only briefly mentioned,
and details are given in the appendix. Additional results on computational complexity and on games
with discrete budgets appear in the full version of this paper


